Building your Cross-Platform Application with RHEEM

Today, organizations typically perform tedious and costly tasks to juggle their code and data across different data processing platforms. Addressing this pain and achieving automatic cross-platform data processing is quite challenging because it requires quite good expertise for all the available data processing platforms. In this report, we present Rheem, a general-purpose cross-platform data processing system that alleviates users from the pain of finding the most efficient data processing platform for a given task. It also splits a task into subtasks and assigns each subtask to a specific platform to minimize the overall cost (e.g., runtime or monetary cost). To offer cross-platform functionality, it features (i) a robust interface to easily compose data analytic tasks; (ii) a novel cost-based optimizer able to find the most efficient platform in almost all cases; and (iii) an executor to efficiently orchestrate tasks over different platforms. As a result, it allows users to focus on the business logic of their applications rather than on the mechanics of how to compose and execute them. Rheem is released under an open source license.

==> rheem.tex <==
%!TEX root = main.tex

% Let us first start with what \rheem is {\em not}.
First of all, let us emphasize that \rheem is \emph{not} yet another data processing platform.
On the contrary, it is designed to work as a middleware between applications and data processing platforms, helping applications to choose the right platform for a given task.
It operates in settings where multiple platforms co-exist and applications should dynamically leverage the full potential of the platforms.
%To our knowledge, 
\rheem is the first general-purpose cross-platform system that alleviates users from the intricacies of the underlying platforms and let them focus on the logic of their applications.

\begin{figure}[h!]
	\vspace{-0.2cm}
	\centering
	\includegraphics[scale=0.175]{figures/architecture.pdf}
	\caption{\rheem's ecosystem and architecture.}
	\label{figure:rheem}
	\vspace{-0.3cm}
\end{figure}

%\rheem is an open source system with an active community. All the components we describe in this paper are available in the latest release (v0.3.0)\footnote{A new release (v.0.4.0) is scheduled for February 2018.}.
%In the following, let us first provide a high-level overview of \rheem to understand its overall design and functionalities.
Figure~\ref{figure:rheem} depicts the \rheem ecosystem, \ie~the \rheem core architecture together with four main applications and several platform drivers.
%both the \rheem ecosystem and the \rheem core architecture.
%The \rheem ecosystem is composed of four main applications: ML4all  -- a machine learning system, BigDansing  -- a data cleaning system--, xDB -- a cross-platform data management system--, and \rheem Studio -- a visual IDE.
%\seb{I find it strange to call applications an ecosystem -- in particular, because an ecosystem is something closd. Also, we have already described the applications above, so I would leave out that point completely.} 
% \jorge{correct, but do you it really hurts to keep them here too for completeness?}
The \rheem core architecture comprises the {\em cross-platform optimizer}, the {\em executor}, the {\em monitor}, the {\em progressive optimizer}, and the {\em cost learner}.
%the \rheem core (\ie~the {\em cross-platform optimizer}, {\em executor}, {\em monitor}, {\em progressive optimizer}, and {\em cost learner} components), and several drivers to support the different platforms.

We briefly explain each of these components in the following and then dive into more details in the next two sections.


\myparagraph{Data and Processing Model}
Users provide a \rheem~{\em plan} to the system (Step~(1) in Figure~\ref{figure:rheem}), using the Java, Scala, RheemLatin, or REST API.
They can also compose their \rheem plan by simply drawing it in the Studio.
%directly code their \rheem plans by using either a native API (Java or Scala) or the data-flow query language (RheemLatin), but also by drawing the plan in the \rheem Studio.
%We  present further details on how to compose a \rheem plan in Section~\ref{section:interfaces}.
%We describe all these three ways in Section~\ref{section:interfaces}.
A \rheem plan is a directed acyclic data flow graph (DAG) whose vertices are {\em \rheem operators} and whose edges represent data flows among the operators.
Specific \op{Loop} operators furthermore accept feedback edges, which allows to express iterative data flows.
The atomic processing units flowing through the plan are called {\em data quanta} and can express a large spectrum of data formats, such as database tuples, edges in a graph, or documents.
The \rheem operators are platform-agnostic and define a particular kind of data transformation over their input data quanta, \eg~a \op{Map} operator transforms individual data quanta while a \op{Reduce} operator aggregates all input data quanta into a single output data quantum.
Conceptually, data quanta are flowing from source operators through the graph, thereby being manipulated in the operators, until they reach a sink operator.
Users can further refine the behavior of operators with \emph{user-defined functions (UDFs)}, such as a transformation or aggregation function. All these render \rheem plans highly expressive in contrast to other cross-platform systems~\cite{gog2015musketeer,ires-bigdata}.

\begin{figure}[h!]
	\vspace{-0.2cm}
	\centering
	\includegraphics[scale=0.17]{figures/plan.pdf}
	\caption{K-means example.}
	\label{figure:plan}
	\vspace{-0.3cm}
\end{figure}

\vspace{-0.2cm}
\begin{example}
Figure~\ref{figure:plan}(a) shows a \rheem plan for k-means.
Initially, the dataset containing the data points is read via a \op{TextFileSource} operator and parsed using a \op{Map} operator while the initial centroids are read via a \op{Collection} source operator.
After the \op{RepeatLoop} operator, the centroids are fed to the \op{Map} operator, where each data point is assigned to the closest centroid.
Notice that as \op{Map} receives the input data points from its default input port, \op{RepeatLoop} has to broadcast the centroids at each iteration to \op{Map} (denoted by the dotted line).
Then, the \op{ReduceBy} operator groups the points that belong to the same centroid and computes their sum and count.
The next \op{Map} operator computes the new centroids by averaging the sum and count.
This process is repeated until the loop condition is satisfied.
The resulting centroids are output in a collection sink.
\end{example}
\vspace{-0.2cm}

\myparagraph{From a \rheem Plan to an Execution Plan}
Given a \rheem plan as input, the cross-platform optimizer produces an {\em execution plan} by selecting one or more of the available platforms to efficiently execute the input plan (Step~(2) in Figure~\ref{figure:rheem}).
For this purpose, it maps the \rheem operators to {\em execution operators}, \ie~operators in \rheem having platform-specific code, using flexible $m$-to-$n$ mappings.
%Supporting $m$-to-$n$ 
Supporting such mappings is particularly useful as it allows to map whole subplans of \rheem operators to subplans of \rheem or execution operators.
As a result, we  can handle different abstraction levels among platforms, \eg~to emulate \rheem operators that are not natively supported by a platform. This is not possible in other systems, such as~\cite{ires-bigdata}.
%Although users can provide their own mappings at any time, \rheem comes with default mappings for most common platforms.

\begin{figure}[h!]
	\vspace{-0.2cm}
	\centering
	\includegraphics[scale=0.17]{figures/mappings.pdf}
	\caption{Operator mappings.}
	\label{figure:mappings}
	\vspace{-0.3cm}
\end{figure}

Figure~\ref{figure:mappings} illustrates the mapping for the \op{ReduceBy} \rheem operator.
The \op{ReduceBy} \rheem operator directly maps to the \op{ReduceBy} Spark execution operator via a 1-to-1 mapping (mapping~(a)).
However, it does not have a direct mapping to a JavaStreams execution operator.
Instead, it maps to a set of \rheem operators (\op{GroupBy} and \op{Map} \rheem operators) via a 1-to-n mapping (mapping~(b)) and vice-versa (mapping~(c)).
In turn, this set of \rheem operators maps to a set of JavaStreams execution operators (\op{GroupBy} and \op{Map} JavaStream execution operators) via an m-to-n mapping (mapping~(d)).
Eventually, these mappings form the search space of execution plans from which \rheem determines the most promising plan alternative according to its cost model.
The cost can be any user-specified cost, \eg~runtime or monetary cost.
The resulting execution plan is again a data flow graph, where
the vertices are now execution operators. An execution plan may comprise additional execution operators for data movement or for reusing data.
%We present in more de tail the optimization process in Section~\ref{section:core}.
%\seb{I would remove the details regarding the mappings. This is probably the least interesting part of the whole optimization process.}\seb{Subsection?}
%\jorge{I believe the mappings allows us to easily plug new platforms. So as we claim ease of use here and there, we might give some details about the features that allow us to do so.}

\vspace{-0.2cm}
\begin{example}
Figure~\ref{figure:plan}(b) shows the k-means execution plan produced by \rheem when Spark and JavaStreams are the only available platforms.
This execution plan exploits high parallelism for the large dataset of input data points and avoids the extra overhead incurred by big data processing platforms for the smaller collection of centroids.
Note that the execution plan also contains three execution operators for transferring (\op{Broadcast}, \op{Collect}) and making data quanta reusable across the platforms (\op{Cache}).
\end{example}
\vspace{-0.2cm}

\myparagraph{Running an Execution Plan}
Four main components contribute to running the execution plan: the executor, the platform drivers, the monitor and the progressive optimizer.
The executor orchestrates the execution of the generated execution plan on the selected platforms (Step~(3) in Figure~\ref{figure:rheem}).
For this, \rheem has a decoupled platform-specific driver for each available platform.
This design choice makes our system very easy to extend to new platforms or update to newer versions of platforms.
During execution, the monitor checks the health of the execution plan and collects statistics to improve the cost model of the optimizer (Step~(4)).
At the same time, the progressive optimizer
%\seb{What about ``progressive optimization'' rather than ``progressive optimizer''? I find it more elegant to have fewer components in the explanation.} 
%\jorge{If we modify this then we will have to modify in several places of the paper, including the architecture figure. We really want to do so?}
is responsible for verifying whether the system needs to change the current execution plan on-the-fly, for example, in case of bad cardinality estimates.
If so it passes the new execution plan to the executor (Step~(5)).

\myparagraph{Offline cost learning}
\rheem also comes with a offline cost learner tool to help users in finding the right cost model for their \rheem installations.
This tool {\em learns} the cost of execution operators from execution logs, which can be either from real executions or generated by our system.
%measures the real execution times from actual execution logs and use the gathered information to {\em learn} the cost functions of each execution operator.
%We provide further explanations in Section~\ref{section:core}.

\myparagraph{Extensibility}
We have designed \rheem to address extensibility as a first-class citizen rather than as ``nice-to-have'' feature.
%This is because operating in an environment where multiple systems co-exist is hard to 
%This is because data science in general is domain specific.
% and hence users must be able to customize their environments according to their needs.
%Users can add new (i)~\rheem and execution operators, including data movement operators, (ii)~operators mappings, and (iii)~platform drivers, all without modifying the existing source code.
Users can add new \rheem and execution operators by merely extending or implementing few abstract classes/interfaces. 
%\op{Operator} class and implement the \op{ExecutionOperator} interface for the execution operators.
\rheem provides template classes
%, such as \op{UnaryToUnaryOperator} or \op{SourceOperator}, 
to facilitate the development for different operator types.
%\seb{Too much (technical) detail in my opinion. The crucial point is that you can extend platforms and operators via a plug-in infrastructure. Maybe give a number on how many lines of code an extension needs instead?}
Users can also add operator mappings by simply implementing an interface and specifying a graph pattern that matches the \rheem operator.
Similarly, users can plug new data processing platforms by providing a new driver, besides the execution operators and their mappings.
We have exploited the extensibility of \rheem to boost the performance of our applications  presented in Section~\ref{section:usecases}.
% to adapt \rheem to the domain of each of our applications presented in Section~\ref{section:usecases}.






